MeshDMP: Motion Planning on Discrete Manifolds using Dynamic Movement Primitives

An open problem in industrial automation is to reliably perform tasks requiring in-contact movements with complex workpieces, as current solutions lack the ability to seamlessly adapt to the workpiece geometry. In this paper, we propose a Learning from Demonstration approach that allows a robot manipulator to learn and generalise motions across complex surfaces by leveraging differential mathematical operators on discrete manifolds to embed information on the geometry of the workpiece extracted from triangular meshes, and extend the Dynamic Movement Primitives (DMPs) framework to generate motions on the mesh surfaces. We also propose an effective strategy to adapt the motion to different surfaces, by introducing an isometric transformation of the learned forcing term. The resulting approach, namely MeshDMP, is evaluated both in simulation and real experiments, showing promising results in typical industrial automation tasks like car surface polishing.

==> sections/extras.tex <==


\subsection{Notes}
Let $\mathbb M$ be a smooth manifold parametrised as 
\begin{align*}
    \phi : \mathcal U \subset \mathbb R^n & \rightarrow \mathbb R^m \\
    (u_1, \dots, u_n) & \mapsto \phi(u_1, \dots u_n),
\end{align*}
With the following notation we define the tangent vector yield by the map $\phi$ of the $i$-th coordinate:
\[\partial_ i = \frac{\partial \phi}{\partial u_i}. \]
In this regard, the tangent space $T_p\mathbb M$ of the manifold $\mathbb M$ at the point $p \in \mathbb M$, has as basis the vectors $\{\partial_1, \dots \partial_n\}$.

Given a (pseudo-)Riemaannian metric $\langle \cdot, \cdot \rangle$, the (pseudo-)metric tensor is given by
\[ g_{ij} = \langle \partial_i, \partial_j \rangle.\]
Collecting those coefficients in a "matrix" $G = (g_{ij})$, the inverse elements of the metric tensor (denoted with the super-script) are
\[ g^{ij} = (G^{-1})_{ij}. \]

A curve $\gamma : \mathbb R  \rightarrow \mathbb M$, parametrised in $t$, is a geodesic if and only if it satisfy the following differential equation:
\[ \frac{d^2 u_i}{dt^2} + \Gamma_{jk}^i \frac{du_j}{dt} \frac{du_k}{dt} = 0 \quad \textrm{for all } i =1,\dots,n,\]
where $\Gamma_{jk}^i$ are the Christoffel symbols defined as
\[ \Gamma_{jk}^i = \frac 1 2 g^{li} \left( \frac{\partial g_{lj}}{\partial u_k} + \frac{\partial g_{kl}}{\partial u_j} - \frac{\partial g_{jk}}{\partial u_l} \right). \]
